Physics-Inspired Heuristics for Soft MIMO Detection in 5G New Radio and Beyond

Overcoming the conventional trade-off between throughput and bit error rate (BER) performance, versus computational complexity is a long-term challenge for uplink Multiple-Input Multiple-Output (MIMO) detection in base station design for the cellular 5G New Radio roadmap, as well as in next generation wireless local area networks. In this work, we present ParaMax, a MIMO detector architecture that for the first time brings to bear physics-inspired parallel tempering algorithmic techniques [28, 50, 67] on this class of problems. ParaMax can achieve near optimal maximum-likelihood (ML) throughput performance in the Large MIMO regime, Massive MIMO systems where the base station has additional RF chains, to approach the number of base station antennas, in order to support even more parallel spatial streams. ParaMax is able to achieve a near ML-BER performance up to 160x160 and 80x80 Large MIMO for low-order modulations such as BPSK and QPSK, respectively, only requiring less than tens of processing elements. With respect to Massive MIMO systems, in 12x24 MIMO with 16-QAM at SNR 16 dB, ParaMax achieves 330 Mbits/s near-optimal system throughput with 4--8 processing elements per subcarrier, which is approximately 1.4x throughput than linear detector-based Massive MIMO systems.

==> PMIS.tex <==
\section{ParaMax Ising Solver (PMIS)}
\label{s:PMIS}


\subsection{Principle Algorithm: Parallel Tempering}
\label{s:primer_pt}


Simulated annealing (Section~\ref{s:primer_sa}) guarantees that the spin system
will eventually find the lowest energy spin configurations if the temperature is lowered
slowly enough, but for hard optimization problem it may require an exponentially long time. Indeed,
a rugged energy landscape ``traps'' the spin system in local minima which are hard to escape.
To overcome this problem, Swendsen and Wang devised a technique called ``parallel tempering'' (also
known as replica exchange method) \cite{swendsen1986replica} to help the spin system escaping local minima and thermalize
faster at low temperature. Parallel tempering is one of the most powerful classical optimization techniques 
that has been shown to perform well on a variety of hard optimization problems.\footnote{Parallel tempering is extremely versatile and powerful such that, in many cases,
drastically speedup the thermalization of the spin system \cite{katzgraber2006feedback, young2004absence, trebst2006optimized}, 
including benchmark against quantum annealers \cite{mandra2016strengths, mandra2017exponentially, mandra2018deceptive}.}
The basic principle of parallel tempering is simple: rather than having a ``single'' spin system for
which the temperature is slowly lowered, different ``replicas'' are simulated in parallel, each with
a different temperature. After a certain amount of Metropolis updated, the temperatures of the
two replicas $r_1$ and $r_2$ are ``exchanged'' following the updating rule:
\begin{equation}\label{eq:pt}
    p(r_1 \leftrightarrow r_2) = \min\left\lbrace{1, e^{\Delta\beta\Delta\mathcal{H}}}\right\rbrace,
\end{equation}
with $\Delta\beta$ and $\Delta\mathcal{H}$ being the difference in the inverse of temperature 
and the difference in energies of the two replicas respectively. As one can see, two temperatures
are always exchanged if a replica at higher temperature has a lower energy than a replica
with a lower temperature. Otherwise, the exchange of the two temperatures is either accepted or
rejected accordingly to Eq.~\ref{eq:pt}. Note that parallel tempering is a completely classical algorithm that does not require any specific hardware for its implementation (\emph{cf.} QuAMax requires a quantum hardware).

% As explained in Section~\ref{s:primer_sa} and \ref{s:primer_pt}, 




\subsection{PMIS: Parallel Tempering for ParaMax}
\label{s:pmis_implementation}

The PMIS is the main solver of MIMO detection in the \systemname{} and is based on a highly-optimized simulated annealing featured with \emph{parallel tempering} tailored to optimize Ising models of MLO for MIMO detection. 

% As explained in Section~\ref{s:primer_sa} and \ref{s:primer_pt}, PMIS performs a local search by updating the spin values of a given random initial configuration accordingly to Eq.~\ref{eq:metropolis}. Each replica is associated with a different temperature and temperatures may be exchanged accordingly to the update rule in Eq.~\ref{eq:pt}. Since the calculation of the energy associated to each replica can be trivially reduced to matrix-vector and vector-vector multiplications, PMIS is tailored to maximize the performance for operations involving a relatively small number of spin variables, that is $N_V \lesssim 512$. 
% %
% More precisely, couplings $g_{ij}$ and local fields $f_j$ of the Ising cost
% function $\mathcal{H}$ are stored as a matrix $\mathbf{g}$ and as a vector $\vec{f}$ respectively.
% Therefore, the calculation of $\mathcal{H}$, which is critical for the update
% rules in Eq.~\ref{eq:metropolis} and Eq.~\ref{eq:pt}, is reduced to 
% a matrix-vector multiplication, then followed by a vector multiplication,
% that is:
% \begin{equation}\label{eq:ising-matrix}
%     \mathcal{H}(\vec{s}) = \vec{s} \cdot \left[\mathbf{g} 
%         \cdot \left( \vec{s} + 2\vec{f} \right) \right]/2,
% \end{equation}
% with $\vec{s}$ the vector representing the spin configuration, where the factor $2$ takes into account the symmetry of the matrix $\mathbf{g}$. From Eq.~\ref{eq:ising-matrix}, it is clear that the runtime is proportional to the square of the number of spin variables $N_V$ as shown in Figure~\ref{f:compute_vs_nv}. Therefore, recalling that every replica is independently updated, the overall PMIS runtime scales as $N_V^2 \times N_\text{repl} \times N_{sw}$, with $N_\text{repl}$ and $N_\text{sw}$ the number of replicas and sweeps respectively.
% %


% In the PMIS, there are some controllable parameters that affect the system performance in terms of the quality of solution distribution and compute time.\\

% \subsubsection{Tailoring to MIMO Detection}

\begin{figure}
\includegraphics[width=0.95\linewidth]{figures/UFO_baseline.png}
\caption{Sweep analysis of \systemname{} solving 16-QAM MIMO detection at 20dB SNR: \emph{\textbf{overview (left)}} varying user numbers and \emph{\textbf{detailed view (right)}} at 20-user (\emph{i.e.}, 20$\times$20 MIMO) and 50 sweeps across  instances. In the figures, lines report median, shadings report 10th. and 90th. percentile, and the box plots report  ‘0th.’and ‘99.5th.’ as whiskers, upper/lower quartiles as boxes, and outliers as thin horizontal marks. Each $\times$ symbol reports each instance's corresponding value point.}
\label{f:sweep_opt}
\end{figure}


\begin{figure}
\centering
% \includegraphics[width=\linewidth]{figures/tts_vs_tte.png}
\includegraphics[width=\linewidth]{figures/temp_analysis.png}
\caption{Temperature range analysis of PMIS solving 20-user 16-QAM MIMO detecton at 20dB SNR with required $N_{pe}$ to ML-bound with 99\% confidence, where thick dotted (red) lines highlight the best low and high temperature in terms of the minimum required $N_{pe}$ to ML-bound performance with 99\% confidence. \textcolor{red}{(NEED TO REMOVE BOUNDARY LINE)}}
\label{f:temp_opt}
\end{figure}

% \subsection{ParaMax Implementation}
% \label{s:pmis_implementation}

The PMIS performs a local search by updating the spin values of a given random initial configuration accordingly to Eq.~\ref{eq:metropolis}. Each replica is associated with a different temperature and temperatures may be exchanged accordingly to the update rule in Eq.~\ref{eq:pt}. Since the calculation of the energy associated to each replica can be trivially reduced to matrix-vector and vector-vector multiplications, PMIS is tailored to maximize the performance for operations involving a relatively small number of spin variables, that is $N_V \lesssim 512$. 
%
More precisely, couplings $g_{ij}$ and local fields $f_j$ of the Ising cost
function $\mathcal{H}$ are stored as a matrix $\mathbf{g}$ and as a vector $\vec{f}$ respectively.
Therefore, the calculation of $\mathcal{H}$, which is critical for the update
rules in Eq.~\ref{eq:metropolis} and Eq.~\ref{eq:pt}, is reduced to 
a matrix-vector multiplication, then followed by a vector multiplication,
that is:
\begin{equation}\label{eq:ising-matrix}
    \mathcal{H}(\vec{s}) = \vec{s} \cdot \left[\mathbf{g} 
        \cdot \left( \vec{s} + 2\vec{f} \right) \right]/2,
\end{equation}
with $\vec{s}$ the vector representing the spin configuration, where the factor $2$ takes into account the symmetry of the matrix $\mathbf{g}$. 
% The details of PMIS implementation are in Section~\ref{s:implementation}.

\parahead{Number of replicas.} To reduce the computational cost at the bare minimum, we have opted for a ``bang-bang'' parallel tempering approach. That is, only two replicas are used: one at very low temperature and one at higher temperature: the replica at lower temperature acts as a ``greedy'' searcher while the replica at a higher temperature act as an ``observer''. When the greedy searcher is stack in a local minimum, the two replicas can exchange ``role'' (i.e. temperature) and eventually explore the energy landscape faster. While this has been successfully used in the context of quantum annealing \cite{yang2017optimizing}, this is one of the first reports of a bang-bang parallel tempering schedule for a classical optimization problem.



\parahead{Number of Metropolis Sweeps.} 
%To see an impact of the sweep number,
{\DV{Each PMIS run is parametrized by the number of Metropolis updates of the parallel tempering algorithms. A sequential update of all spins of the instance is a "sweep".}} We examine different number of sweeps from one to 80 with 16-QAM modulation at 20dB SNR in Figure~\ref{f:sweep_opt}, where the \emph{left} part presents overview of analysis for four different MIMO sizes as a function of sweep numbers, while the \emph{right} part provides the detailed view of 20$\times$20 MIMO at 50 sweeps across 20 instances.
Both overview and detailed view consist of detection latency $\mu$s (\emph{top}), probability of finding the ML solution (\emph{middle}), and the required $N_{PE}$ to ML-bound with 99\% confidence (\emph{bottom}). 
% In the overview, each line reports median (50\%) as a function of sweep numbers. In the detailed view, the boxplot (\emph{right, top}) reports latency `0th.' and `99.5th.' as whiskers, upper/lower quartiles as boxes, and thin horizontal marks for outliers across 50 instances. Each $\times$ symbol \emph{(right, middle \& bottom)} reports each instance's corresponding points (showing only 20 to save space), while shading reports 10th. and 90th. percentile.
We observe that as the number of sweeps increases, both runtime and probability of finding the ML solution tend to increase (\emph{i.e.}, the less $N_{PE}$ is required to ML-bound performance at the expense of the longer latency). We choose the number sweeps = 50 as an appropriate point that satisfies both the feasible latency for the current LTE standard and the secure available number of $N_{PE}$ for the recent hardware specification. 
\\


\parahead{Temperature Range.} We analyze the minimum and maximum temperature setting, $T_{min}$ and $T_{max}$ for the PMIS in Figure~\ref{f:temp_opt}. The range from 0.0 to 0.1 with 0.005 interval is tested at 50 sweeps. Unlike the number of sweeps, the temperature range does not influence the \systemnames{} runtimes, so the range is chosen where the system requires the minimum $N_{PE}$ to achieve the ML-bound performance, which is $T_{min}$=0.05 and $T_{max}$=0.06.%\\


==> quantum_annealing.tex <==
\section{Quantum Computation}
\label{s:quantum}


\subsection{Quantum Annealing}
\subsection{Ising Formulation}
FROM SIGCOMM 2019
\paragraph{Ising spin glass form.}  In this form the
solution variables are traditionally referred to as 
\emph{spins} $s_i \in \left\{ +1, -1\right\}$.
\begin{eqnarray}
\hat{s}_1, \ldots, \hat{s}_N = 
    \arg\min_{\left\{ s_1, \ldots, s_N \right\}} \left(\sum^{N}_{i<j} g_{ij} s_i s_j + \sum^{N}_{i} f_i s_i\right)
\label{eqn:ising}
\end{eqnarray}
where $N$ is the number of spin variables,
and $g_{ij}$ and $f_{i}$ are the Ising \emph{model parameters} that 
characterize the problem.
The $f_{i}$ characterize the preference 
for each spin to be $+1$ or $-1$: positive
indicates a preference for $-1$ while negative 
indicates a preference for $+1$, with the magnitude
corresponding to the magnitude of the preference
for either state.
The $g_{ij}$ capture preferred correlations 
between spins: positive causes the QA
to prefer $s_i \neq s_j$, while negative causes
the QA to prefer $s_i = s_j$ in its optimization outcome.
Analogously to $f_i$, the magnitude of $g_{ij}$ corresponds
to the magnitude of its preference.
% \subsection{Quantum Annealing Machine}
% \subsection{Interpretation of input }
% \subsection{Ising Formulation}
% \subsection{Reverse Annealing}


==> reverse_annealing.tex <==
\section{Reverse Annealing}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/cdf_rv_8.png}
\caption{CDF of energy percentile (\emph{Upper}) and bit error number per channel use (\emph{Lower}) out of upto 1,000,000 anneal samples of 20-50 instances of 36-variable decoding problems for different modulations and \textbf{algorithms}: \emph{(Left)} forward annealing or QuAMax, \emph{(Center)}: reverse annealing starting at a randomly picked initial state, \emph{(Right)} reverse annealing starting at the result state of greedy search, which is the simplest linear decoder.}
\label{f:cdf_reverse}
\end{figure}


First, we investigate reverse annealing (RA) to see if improved performance can be achieved compared against forward annealing. For RA, in addition to standard QA parameters such as embedding penalty term, anneal time, and pause location, an initial state at which RA algorithm begins is a key factor that affects the overall performance, which opens a change of quantum-classic hybrid algorithm. A fundamental metric to evaluate sampling-based decoders is a distribution of samples. Figure~\ref{f:cdf_reverse} shows cumulative distribution function (CDF) of energy percentile (upper) and number of bit errors (lower) out of all anneal samples of 36-variable MIMO decoding (36-user BPSK, 18-user QPSK, 9-user 16-QAM, and 6-user 64-QAM) solved by forward annealing and reverse annealing. While the lower energy gap percentile means the closer objective function's value to the ground truth energy which is directly related to euclidean distance in ML detection, the lower number of bit errors means the lower hamming distance against the ground truth state. We observe that RA that begins at a randomly picked state (Figure~\ref{f:cdf_reverse}, \emph{center}) works worse than forward annealing (Figure~\ref{f:cdf_reverse}, \emph{left}) in that CDF of both energy percentile $\Delta E\%$ and number of bit errors tends to be toward right. On the other hand, RA starting at a solution of greedy search (Figure~\ref{f:cdf_reverse}, \emph{right}), which is the simplest decoding scheme in our consideration (simpler than zero-forcing), shows radical improvement. Especially in the case of BPSK and QPSK, all anneal samples find the ground truth successfully, even with the simplest decoder. However, this improvement may not be from reverse annealing itself, since it's already quantum-classic hybrid algorithm. Therefore, we further investigate reverse annealing with some instances in order to understand and evaluate RA itself thoroughly and thus we are able to make full use of advantages of RA for \systemname{}.



\begin{figure}
\centering
\includegraphics[width=0.90\linewidth]{figures/reverse_annealing_analysis_13.png}
\caption{Average energy and success probability out of reverse annealing samples of two 8-user 16-QAM decoding instances across different input energy percentiles $\Delta E^{IS}\%$. Colored parts are a close up of the second instance $\Delta E^{IS}\%$ below 10\%. No data at 0.2\% and 0.4\%.}
\label{f:reverse_initial_state}
\end{figure}

\parahead{Energy percentile of initial state.} For in-depth analysis on reverse annealing, we first try to find a relationship between energy percentile of RA initial state and overall sampling performance. We define $\Delta E\%$, the energy percentile against the ground truth energy before, but we newly define the energy percentile of RA initial state as $\Delta E^{IS}\%$ for distinction, even though its calculation is the exactly same as $\Delta E\%$. Using 100,000 error-case samples with the ground truth state, we obtain corresponding $\Delta E^{IS}\%$ of every different sample state and then we run RA (10,000 anneals or annealing samples per parameter) varying $\Delta E^{IS}\%$, with corresponding states as the RA initial state. Figure~\ref{f:reverse_initial_state} shows success probability and average energy (at fixed JF) out of reverse annealing samples of two 8-user 16-QAM decoding instances across different $\Delta E^{IS}\%$ (interval $\delta = 2\%$) and we also highlight instance 2's $\Delta E^{IS}\%\leq10\%$ with denser interval ($\delta = 0.2\%$). Note that there is no data point at $\Delta E^{IS}\%=0.2\%$ and $=0.4\%$. This means none of the error case states have an energy that is very close (less than 0.4\% difference) to the ground truth one and it is very likely that it does not exist at all for noise-free cases. We observe that while all 10,000 RA samples out of RA run starting at $\Delta E^{IS}\%=0\%$ (\emph{i.e.,} the ground truth state) enable to find the ground truth state, the samples out of RA run starting at $\Delta E^{IS}\%\neq0\%$ achieve less than 1\% of success probability. This implies that the decent success probability ($\Delta E\%=0$ or zero error bit) in Figure~\ref{f:cdf_reverse} (\emph{right}) is achieved largely by the greedy search at least in the case of high modulations such as 16- and 64-QAM. RA run with $\Delta E^{IS}\%\leq4\%$ have at least one sample (out of 10,000 anneal samples) finding the ground truth. Regarding average energy, the lower average energy is obtained for the lower $\Delta E^{IS}\%$ when $\Delta E^{IS}\%\leq 20-30\%$, after which noisy results are obtained.


\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{figures/reverse_pause_20.png}
\caption{Success probability out of reverse annealing samples and TTS of reverse annealing of a 8-user 16-QAM decoding instance with different energy percentiles of initial state $(\Delta E^{IS}\%)$ across different switch and pause locations $(s_p)$.}
\label{f:reverse_pause}
\end{figure}


\parahead{Switch and pause location.} Another important factor in RA that affects sampling performance is switch and pause location $s_p$ ($0 \leq s_p \leq 1$). Recall that RA starts annealing backward from the selected initial state and at some point $s_p$ it stops and switches to annealing forward. The choice of $s_p$ is critical, since if $s_p$ is too high ($\approx 1$) samples are likely to end up being the selected initial state and if $s_p$ is too low ($\approx 0$) the initial state is wiped out which means the main advantage of RA is no longer utilized. When backward annealing reaches $s_p$, we pause the annealing for 1~$\mu$s, since the improvements by anneal pause have been shown even for reverse annealing [REF]. We plot RA's success probability and TTS 99\% across different switch and pause position at fixed JF in Figure~\ref{f:reverse_pause}. The red line denotes the RA run with the ground truth as a RA initial state ($\Delta E^{IS}\% = 0\%$) and each dotted line denotes RA runs at various initial states of $0 < \Delta E^{IS}\% < 10\%$ ($\delta=0.2\%$). The initial states of $\Delta E^{IS}\% \geq 10\%$ are out of our consideration since these states are very less likely to be selected for RA initial state in the system. The best switch and pause position for this instance is $s_p=0.45$ which shows the best median TTS results. Further, the median of best $s_p$ across different 8-user 16-QAM decoding instances will be used for \systemname{}. In the same way, $s_p$ can be chosen for different modulations and user numbers. In the case of FA for the same instance, at most of $s_p$ it fails to find the ground truth. RA can achieve a slightly better performance than FA. However, note that TTS performance of reverse annealing is not good enough for wireless MIMO decoding, when $\Delta E^{IS}\% \neq 0\%$. For this reason, the pre-decision process that might be able to make the problems simpler is required, whose performance will be discussed x.              

